A Sample of Type II-L Supernovae

What are Type II-Linear supernovae (SNe II-L)? This class, which has been ill defined for decades, now receives significant attention -- both theoretically, in order to understand what happens to stars in the ~15-25Mo range, and observationally, with two independent studies suggesting that they cannot be cleanly separated photometrically from the regular hydrogen-rich SNe II-P characterised by a marked plateau in their light curve. Here, we analyze the multi-band light curves and extensive spectroscopic coverage of a sample of 35 SNe II and find that 11 of them could be SNe II-L. The spectra of these SNe are hydrogen deficient, typically have shallow Halpha absorption, may show indirect signs of helium via strong OI 7774 absorption, and have faster line velocities consistent with a thin hydrogen shell. The light curves can be mostly differentiated from those of the regular, hydrogen-rich SNe II-P by their steeper decline rates and higher luminosity, and we propose as a defining photometric characteristic the decline in the V band: SNe II-L seem to decline by more than 0.5 mag from peak brightness by day 50 after explosion. Using our sample we provide template light curves for SNe II-L and II-P in 4 photometric bands.

==> phot_fullp2.tex <==

 
\begin{table*}
\caption{Full light curves\label{t:phot}}
\begin{tabular}{ccccccc}
\hline\hline
SN name &
MJD &
Age \tablenotemark{a} &
B($\sigma_B$) &
V($\sigma_V$) &
R($\sigma_R$) &
I($\sigma_I$)\\
\hline
1999co	  & 51352.42	 & 20.4	& 17.975(0.053)	 & 17.663(0.056)	 & --	 & 17.275(0.125) \\ 
1999co	  & 51370.38	 & 38.4	& 18.472(0.132)	 & 17.927(0.044)	 & --	 & 17.318(0.112) \\ 
1999co	  & 51377.41	 & 45.4	& 18.612(0.082)	 & 18.011(0.060)	 & --	 & 17.403(0.095) \\ 
1999co	  & 51384.35	 & 52.4	& 18.831(0.228)	 & 18.132(0.218)	 & --	 & 17.637(0.194) \\ 
1999co	  & 51391.40	 & 59.4	& 18.925(0.139)	 & 18.197(0.115)	 & --	 & 17.501(0.112) \\ 
1999co	  & 51398.30	 & 66.3	& 19.148(0.173)	 & 18.360(0.142)	 & --	 & 17.567(0.187) \\ 
1999co	  & 51405.29	 & 73.3	& 19.335(0.143)	 & 18.451(0.115)	 & --	 & 17.551(0.128) \\ 
1999co	  & 51412.23	 & 80.2	& 19.285(0.250)	 & 18.473(0.084)	 & --	 & 18.033(0.230) \\ 
1999co	  & 51419.30	 & 87.3	& 19.532(0.340)	 & 18.490(0.138)	 & --	 & 17.608(0.136) \\ 
1999co	  & 51426.23	 & 94.2	& 19.683(0.184)	 & 18.840(0.102)	 & --	 & 17.788(0.156) \\ 
1999co	  & 51433.20	 & 101.2	& 19.799(0.274)	 & 19.182(0.147)	 & --	 & 17.938(0.165) \\ 
2000dc	  & 51766.25	 & 4.4	& 16.631(0.032)	 & 16.461(0.025)	 & 16.288(0.023)	 & 16.045(0.042) \\ 
2000dc	  & 51767.22	 & 5.4	& 16.538(0.027)	 & 16.372(0.026)	 & 16.120(0.017)	 & 15.881(0.036) \\ 
2000dc	  & 51773.24	 & 11.4	& 16.460(0.034)	 & 16.150(0.019)	 & 15.846(0.012)	 & 15.505(0.030) \\ 
2000dc	  & 51775.30	 & 13.5	& 16.460(0.031)	 & 16.180(0.021)	 & 15.826(0.019)	 & 15.533(0.032) \\ 
2000dc	  & 51777.27	 & 15.5	& 16.545(0.024)	 & 16.198(0.021)	 & 15.878(0.016)	 & 15.580(0.025) \\ 
2000dc	  & 51779.21	 & 17.4	& 16.613(0.031)	 & 16.253(0.015)	 & 15.914(0.016)	 & 15.598(0.035) \\ 
2000dc	  & 51781.23	 & 19.4	& 16.712(0.024)	 & 16.288(0.017)	 & 15.908(0.010)	 & 15.637(0.036) \\ 
2000dc	  & 51783.21	 & 21.4	& 16.804(0.027)	 & 16.264(0.020)	 & 15.925(0.016)	 & 15.629(0.037) \\ 
2000dc	  & 51785.21	 & 23.4	& 16.872(0.027)	 & 16.315(0.019)	 & 15.914(0.015)	 & 15.625(0.031) \\ 
2000dc	  & 51787.19	 & 25.4	& 17.025(0.048)	 & 16.375(0.017)	 & 15.960(0.014)	 & 15.663(0.030) \\ 
2000dc	  & 51790.21	 & 28.4	& 17.196(0.045)	 & 16.457(0.019)	 & 15.979(0.016)	 & 15.705(0.033) \\ 
2000dc	  & 51792.21	 & 30.4	& 17.410(0.042)	 & 16.475(0.023)	 & 16.031(0.018)	 & 15.712(0.034) \\ 
2000dc	  & 51794.20	 & 32.4	& 17.492(0.073)	 & 16.547(0.018)	 & 16.079(0.024)	 & 15.747(0.037) \\ 
2000dc	  & 51801.19	 & 39.4	& --	 & 16.877(0.101)	 & 16.211(0.056)	 & 15.883(0.079) \\ 
2000dc	  & 51804.16	 & 42.4	& 18.106(0.096)	 & 16.921(0.060)	 & 16.279(0.024)	 & 15.865(0.066) \\ 
2000dc	  & 51807.18	 & 45.4	& 18.101(0.112)	 & 16.967(0.043)	 & 16.327(0.019)	 & 15.953(0.052) \\ 
2000dc	  & 51812.21	 & 50.4	& 18.458(0.096)	 & 17.085(0.039)	 & 16.396(0.023)	 & 16.053(0.053) \\ 
2000dc	  & 51816.14	 & 54.3	& 18.526(0.120)	 & 17.100(0.047)	 & 16.482(0.037)	 & 16.032(0.064) \\ 
2000dc	  & 51820.17	 & 58.4	& 18.619(0.142)	 & 17.208(0.036)	 & 16.487(0.026)	 & 16.107(0.048) \\ 
2000dc	  & 51831.13	 & 69.3	& 18.625(0.143)	 & 17.463(0.074)	 & 16.657(0.038)	 & 16.203(0.069) \\ 
2000dc	  & 51839.12	 & 77.3	& 18.730(0.189)	 & 17.420(0.089)	 & 16.677(0.044)	 & 16.273(0.120) \\ 
2001cy	  & 52091.44	 & 6.4	& 15.918(0.026)	 & 15.958(0.021)	 & 15.828(0.017)	 & 15.779(0.037) \\ 
2001cy	  & 52092.48	 & 7.5	& 15.988(0.030)	 & 15.809(0.018)	 & 15.817(0.014)	 & 15.738(0.029) \\ 
2001cy	  & 52093.44	 & 8.4	& 15.967(0.042)	 & 15.976(0.036)	 & 15.841(0.044)	 & 15.770(0.034) \\ 
2001cy	  & 52094.38	 & 9.4	& 15.993(0.043)	 & 15.968(0.032)	 & 15.823(0.033)	 & 15.781(0.036) \\ 
2001cy	  & 52095.40	 & 10.4	& 16.041(0.080)	 & 15.932(0.052)	 & 15.845(0.025)	 & 15.757(0.023) \\ 
2001cy	  & 52096.41	 & 11.4	& 16.083(0.040)	 & 16.013(0.021)	 & 15.865(0.021)	 & 15.811(0.026) \\ 
2001cy	  & 52097.43	 & 12.4	& 16.060(0.076)	 & 16.061(0.035)	 & 15.845(0.077)	 & 15.783(0.184) \\ 
2001cy	  & 52098.38	 & 13.4	& 16.090(0.047)	 & 16.013(0.027)	 & 15.862(0.021)	 & 15.826(0.030) \\ 
2001cy	  & 52099.38	 & 14.4	& 16.165(0.032)	 & 16.006(0.026)	 & 15.882(0.018)	 & 15.831(0.038) \\ 
2001cy	  & 52101.45	 & 16.5	& 16.363(0.041)	 & 16.059(0.032)	 & 15.880(0.024)	 & 15.820(0.023) \\ 
2001cy	  & 52103.39	 & 18.4	& 16.400(0.030)	 & 16.103(0.023)	 & 15.909(0.016)	 & 15.863(0.015) \\ 
2001cy	  & 52105.40	 & 20.4	& 16.657(0.038)	 & 16.186(0.060)	 & 15.960(0.015)	 & 15.906(0.030) \\ 
2001cy	  & 52111.40	 & 26.4	& 17.066(0.047)	 & 16.358(0.024)	 & 16.046(0.014)	 & 15.962(0.030) \\ 
2001cy	  & 52116.37	 & 31.4	& 17.302(0.056)	 & 16.522(0.022)	 & 16.152(0.024)	 & 16.062(0.033) \\ 
2001cy	  & 52121.36	 & 36.4	& 17.509(0.088)	 & 16.617(0.051)	 & 16.244(0.018)	 & 16.069(0.030) \\ 
2001cy	  & 52131.32	 & 46.3	& 17.873(0.091)	 & 16.774(0.051)	 & 16.319(0.021)	 & 16.132(0.028) \\ 
2001cy	  & 52136.36	 & 51.4	& 17.967(0.085)	 & 16.798(0.035)	 & 16.318(0.022)	 & 16.124(0.030) \\ 
2001cy	  & 52141.31	 & 56.3	& 18.104(0.119)	 & 16.837(0.023)	 & 16.445(0.021)	 & 16.173(0.026) \\ 
2001cy	  & 52146.28	 & 61.3	& 18.255(0.112)	 & 16.910(0.036)	 & 16.407(0.024)	 & 16.194(0.031) \\ 
2001cy	  & 52151.26	 & 66.3	& 18.232(0.131)	 & 16.942(0.041)	 & --	 & 16.229(0.025) \\ 
2001cy	  & 52156.34	 & 71.3	& 17.888(0.156)	 & 17.027(0.050)	 & 16.434(0.030)	 & 16.255(0.034) \\ 
2001cy	  & 52161.31	 & 76.3	& 18.534(0.166)	 & 17.025(0.051)	 & 16.442(0.030)	 & 16.233(0.025) \\ 
2001cy	  & 52166.22	 & 81.2	& 18.413(0.101)	 & 17.034(0.033)	 & 16.458(0.016)	 & 16.230(0.025) \\ 
2001cy	  & 52171.22	 & 86.2	& 18.731(0.148)	 & 17.066(0.034)	 & 16.496(0.019)	 & 16.318(0.024) \\ 
2001cy	  & 52176.19	 & 91.2	& 18.595(0.094)	 & 17.179(0.034)	 & 16.525(0.032)	 & 16.385(0.020) \\ 
2001cy	  & 52181.18	 & 96.2	& 18.908(0.152)	 & 17.343(0.037)	 & 16.614(0.021)	 & 16.376(0.033) \\ 
2001cy	  & 52186.19	 & 101.2	& 18.999(0.147)	 & 17.449(0.041)	 & 16.734(0.024)	 & 16.539(0.035) \\ 
2001do	  & 52136.25	 & 3.1	& 16.127(0.030)	 & 15.924(0.022)	 & 15.719(0.016)	 & 15.618(0.020) \\ 
2001do	  & 52137.27	 & 4.1	& 16.187(0.039)	 & 15.898(0.017)	 & 15.665(0.013)	 & 15.521(0.020) \\ 
2001do	  & 52138.24	 & 5.0	& 16.174(0.031)	 & 15.828(0.017)	 & 15.615(0.016)	 & 15.432(0.016) \\ 
2001do	  & 52139.23	 & 6.0	& 16.160(0.022)	 & 15.849(0.023)	 & 15.554(0.013)	 & 15.386(0.016) \\ 
2001do	  & 52140.24	 & 7.0	& 16.150(0.024)	 & 15.834(0.016)	 & 15.548(0.017)	 & 15.356(0.018) \\ 
2001do	  & 52141.25	 & 8.1	& 16.220(0.027)	 & 15.833(0.021)	 & 15.537(0.017)	 & 15.329(0.020) \\ 
2001do	  & 52144.22	 & 11.0	& 16.248(0.023)	 & 15.825(0.014)	 & 15.505(0.014)	 & 15.260(0.021) \\ 
2001do	  & 52147.21	 & 14.0	& 16.363(0.032)	 & 15.869(0.016)	 & 15.508(0.023)	 & 15.212(0.017) \\ 
2001do	  & 52150.22	 & 17.0	& 16.505(0.039)	 & 15.961(0.019)	 & 15.558(0.015)	 & 15.332(0.023) \\ 
2001do	  & 52153.22	 & 20.0	& 16.554(0.035)	 & 16.010(0.027)	 & 15.600(0.020)	 & 15.312(0.023) \\ 
2001do	  & 52156.22	 & 23.0	& 16.783(0.052)	 & 16.095(0.020)	 & 15.629(0.016)	 & 15.366(0.021) \\ 
2001do	  & 52159.19	 & 26.0	& 16.935(0.040)	 & 16.129(0.021)	 & 15.681(0.017)	 & 15.396(0.020) \\ 
2001do	  & 52162.20	 & 29.0	& 17.113(0.045)	 & 16.207(0.026)	 & 15.706(0.020)	 & 15.402(0.020) \\ 
2001do	  & 52165.18	 & 32.0	& 17.334(0.030)	 & 16.310(0.019)	 & 15.759(0.020)	 & 15.428(0.018) \\ 
2001do	  & 52168.18	 & 35.0	& 17.478(0.042)	 & 16.383(0.020)	 & 15.815(0.015)	 & 15.511(0.018) \\ 
2001do	  & 52171.14	 & 37.9	& 17.671(0.045)	 & 16.480(0.020)	 & 15.890(0.014)	 & 15.575(0.020) \\ 
2001do	  & 52174.16	 & 41.0	& 17.813(0.033)	 & 16.575(0.022)	 & 15.927(0.014)	 & 15.617(0.020) \\ 
2001do	  & 52180.14	 & 46.9	& 18.017(0.081)	 & 16.731(0.028)	 & 16.093(0.019)	 & 15.702(0.024) \\ 
2001do	  & 52183.18	 & 50.0	& 18.145(0.135)	 & 16.759(0.032)	 & 16.111(0.019)	 & 15.746(0.026) \\ 
2001do	  & 52186.12	 & 52.9	& 18.267(0.090)	 & 16.883(0.025)	 & 16.162(0.021)	 & 15.769(0.024) \\ 
2001do	  & 52189.12	 & 55.9	& 18.425(0.078)	 & 16.929(0.031)	 & 16.252(0.014)	 & 15.839(0.021) \\ 
2001do	  & 52192.14	 & 58.9	& 18.476(0.056)	 & 16.952(0.019)	 & 16.308(0.018)	 & 15.866(0.023) \\ 
2001do	  & 52197.11	 & 63.9	& 18.579(0.100)	 & 17.075(0.033)	 & 16.307(0.015)	 & 15.922(0.022) \\ 
2001do	  & 52202.10	 & 68.9	& 18.765(0.146)	 & 17.190(0.041)	 & 16.408(0.030)	 & -- \\ 
2001fa	  & 52202.35	 & 4.5	& 16.070(0.014)	 & 16.185(0.014)	 & 16.157(0.018)	 & 16.190(0.020) \\ 
2001fa	  & 52203.34	 & 5.4	& 16.012(0.012)	 & 16.122(0.011)	 & 16.070(0.012)	 & 16.039(0.014) \\ 
2001fa	  & 52204.36	 & 6.5	& 16.051(0.013)	 & 16.067(0.010)	 & 15.996(0.016)	 & 15.955(0.011) \\ 
2001fa	  & 52205.34	 & 7.4	& 16.050(0.023)	 & 16.037(0.013)	 & 15.960(0.015)	 & 15.884(0.022) \\ 
2001fa	  & 52206.36	 & 8.5	& 16.096(0.013)	 & 16.011(0.019)	 & 15.930(0.014)	 & 15.844(0.017) \\ 
2001fa	  & 52207.29	 & 9.4	& 16.210(0.016)	 & 16.055(0.017)	 & 15.912(0.014)	 & 15.868(0.024) \\ 
2001fa	  & 52208.35	 & 10.5	& 16.226(0.027)	 & 16.124(0.016)	 & 15.982(0.014)	 & 15.830(0.021) \\ 
2001fa	  & 52209.36	 & 11.5	& 16.321(0.024)	 & 16.157(0.026)	 & 15.999(0.029)	 & -- \\ 
2001fa	  & 52217.24	 & 19.3	& 16.931(0.030)	 & 16.568(0.024)	 & 16.364(0.019)	 & 16.144(0.025) \\ 
2001fa	  & 52218.25	 & 20.4	& 17.046(0.031)	 & 16.752(0.019)	 & 16.468(0.017)	 & 16.274(0.027) \\ 
2001fa	  & 52219.39	 & 21.5	& 17.132(0.074)	 & 16.807(0.036)	 & --	 & 16.382(0.093) \\ 
2001fa	  & 52221.33	 & 23.4	& 17.236(0.059)	 & 16.870(0.024)	 & 16.567(0.021)	 & 16.380(0.023) \\ 
2001fa	  & 52223.32	 & 25.4	& 17.461(0.038)	 & 16.985(0.015)	 & 16.696(0.015)	 & 16.496(0.028) \\ 
2001fa	  & 52228.32	 & 30.4	& 17.782(0.032)	 & 17.148(0.020)	 & 16.771(0.015)	 & 16.629(0.038) \\ 
2001fa	  & 52231.29	 & 33.4	& 18.000(0.044)	 & 17.181(0.025)	 & 16.819(0.021)	 & 16.595(0.020) \\ 
2001fa	  & 52250.27	 & 52.4	& 18.421(0.056)	 & 17.394(0.032)	 & 16.937(0.023)	 & 16.797(0.037) \\ 
2001fa	  & 52278.20	 & 80.3	& --	 & 18.814(0.099)	 & 18.230(0.072)	 & 17.964(0.053) \\ 
2001fa	  & 52283.14	 & 85.2	& --	 & 18.859(0.116)	 & 18.436(0.197)	 & 18.008(0.198) \\ 
2001fa	  & 52288.19	 & 90.3	& --	 & 19.131(0.283)	 & 18.423(0.106)	 & 18.196(0.093) \\ 
2001fa	  & 52293.10	 & 95.2	& --	 & 19.814(0.209)	 & 18.657(0.101)	 & 18.516(0.116) \\ 
2003hf	  & 52866.23	 & 3.0	& 17.910(0.036)	 & 18.166(0.054)	 & 18.226(0.039)	 & 18.136(0.086) \\ 
2003hf	  & 52867.17	 & 4.0	& 17.591(0.025)	 & 17.874(0.030)	 & 17.882(0.024)	 & 17.900(0.080) \\ 
2003hf	  & 52868.17	 & 5.0	& 17.447(0.018)	 & 17.752(0.029)	 & 17.720(0.030)	 & 17.717(0.066) \\ 
2003hf	  & 52869.17	 & 6.0	& 17.414(0.029)	 & 17.577(0.021)	 & 17.596(0.024)	 & 17.548(0.043) \\ 
2003hf	  & 52870.17	 & 7.0	& 17.358(0.017)	 & 17.501(0.025)	 & 17.448(0.017)	 & 17.405(0.031) \\ 
2003hf	  & 52871.17	 & 8.0	& 17.326(0.024)	 & 17.414(0.022)	 & 17.380(0.016)	 & 17.257(0.077) \\ 
2003hf	  & 52872.17	 & 9.0	& 17.301(0.017)	 & 17.370(0.022)	 & 17.275(0.017)	 & 17.262(0.046) \\ 
2003hf	  & 52873.17	 & 10.0	& --	 & 17.317(0.022)	 & 17.284(0.027)	 & 17.126(0.068) \\ 
2003hf	  & 52874.16	 & 11.0	& 17.252(0.021)	 & 17.251(0.022)	 & 17.167(0.027)	 & 17.071(0.037) \\ 
2003hf	  & 52875.19	 & 12.0	& 17.239(0.017)	 & 17.250(0.018)	 & 17.125(0.025)	 & 17.041(0.040) \\ 
2003hf	  & 52876.17	 & 13.0	& 17.264(0.022)	 & 17.213(0.027)	 & 17.098(0.021)	 & 17.033(0.040) \\ 
2003hf	  & 52878.16	 & 15.0	& 17.324(0.020)	 & 17.234(0.022)	 & 17.101(0.016)	 & 16.990(0.038) \\ 
2003hf	  & 52879.18	 & 16.0	& 17.349(0.019)	 & 17.259(0.023)	 & 17.109(0.022)	 & 16.964(0.035) \\ 
2003hf	  & 52880.18	 & 17.0	& 17.406(0.021)	 & 17.274(0.015)	 & 17.128(0.023)	 & 16.977(0.032) \\ 
2003hf	  & 52883.15	 & 20.0	& 17.574(0.029)	 & 17.324(0.021)	 & 17.162(0.024)	 & 17.020(0.030) \\ 
2003hf	  & 52885.15	 & 22.0	& 17.720(0.080)	 & 17.435(0.025)	 & 17.205(0.043)	 & -- \\ 
2003hf	  & 52887.15	 & 24.0	& 17.853(0.050)	 & 17.473(0.024)	 & 17.257(0.028)	 & 17.072(0.038) \\ 
2003hf	  & 52889.15	 & 26.0	& 17.987(0.038)	 & 17.606(0.030)	 & 17.378(0.023)	 & 17.089(0.029) \\ 
2003hf	  & 52891.15	 & 28.0	& 18.035(0.055)	 & 17.704(0.062)	 & 17.482(0.037)	 & 17.207(0.053) \\ 
2003hf	  & 52893.15	 & 30.0	& 18.301(0.041)	 & 17.871(0.046)	 & 17.530(0.039)	 & 17.343(0.063) \\ 
2003hf	  & 52895.15	 & 32.0	& 18.529(0.055)	 & 17.900(0.053)	 & 17.658(0.031)	 & 17.395(0.040) \\ 
2003hf	  & 52897.15	 & 34.0	& 18.547(0.049)	 & 17.982(0.032)	 & 17.748(0.043)	 & 17.449(0.046) \\ 
2003hf	  & 52899.15	 & 36.0	& 18.713(0.073)	 & 18.129(0.047)	 & 17.754(0.067)	 & 17.466(0.062) \\ 
2003hf	  & 52901.14	 & 37.9	& 18.927(0.069)	 & 18.140(0.037)	 & 17.805(0.043)	 & 17.421(0.050) \\ 
2003hf	  & 52903.14	 & 39.9	& 18.912(0.068)	 & 18.302(0.036)	 & 17.867(0.049)	 & 17.647(0.058) \\ 
2003hf	  & 52905.14	 & 41.9	& 19.180(0.117)	 & 18.343(0.056)	 & 17.942(0.038)	 & 17.627(0.061) \\ 
2003hf	  & 52909.13	 & 45.9	& 19.425(0.134)	 & 18.384(0.052)	 & 17.986(0.029)	 & 17.666(0.060) \\ 
2003hf	  & 52912.13	 & 48.9	& 19.346(0.102)	 & 18.396(0.056)	 & 17.993(0.057)	 & 17.648(0.066) \\ 
2003hf	  & 52915.12	 & 51.9	& --	 & 18.362(0.068)	 & --	 & 17.695(0.101) \\ 
2003hf	  & 52918.12	 & 54.9	& 19.726(0.192)	 & 18.590(0.090)	 & 18.173(0.063)	 & 17.877(0.064) \\ 
2003hk	  & 52872.49	 & 13.0	& 17.020(0.020)	 & 16.999(0.021)	 & 16.832(0.016)	 & 16.764(0.023) \\ 
2003hk	  & 52874.50	 & 15.0	& 17.069(0.021)	 & 16.974(0.019)	 & 16.797(0.021)	 & 16.684(0.029) \\ 
2003hk	  & 52876.51	 & 17.0	& 17.122(0.020)	 & 17.027(0.017)	 & 16.880(0.021)	 & 16.659(0.029) \\ 
2003hk	  & 52879.50	 & 20.0	& 17.192(0.024)	 & 17.080(0.023)	 & 16.940(0.018)	 & 16.659(0.040) \\ 
2003hk	  & 52880.47	 & 21.0	& 17.284(0.023)	 & 17.186(0.025)	 & 16.985(0.018)	 & 16.755(0.028) \\ 
2003hk	  & 52882.50	 & 23.0	& 17.390(0.033)	 & 17.267(0.023)	 & 16.996(0.016)	 & 16.822(0.025) \\ 
2003hk	  & 52884.50	 & 25.0	& 17.478(0.033)	 & 17.325(0.029)	 & 17.076(0.019)	 & 16.991(0.027) \\ 
2003hk	  & 52886.49	 & 27.0	& 17.622(0.030)	 & 17.337(0.024)	 & 17.096(0.019)	 & 16.986(0.025) \\ 
2003hk	  & 52888.48	 & 29.0	& 17.694(0.042)	 & --	 & 17.072(0.024)	 & 17.044(0.093) \\ 
2003hk	  & 52892.44	 & 32.9	& 18.044(0.115)	 & 17.513(0.092)	 & 17.195(0.023)	 & 17.072(0.039) \\ 
2003hk	  & 52899.50	 & 40.0	& 18.225(0.076)	 & --	 & 17.284(0.091)	 & -- \\ 
2003hk	  & 52902.43	 & 42.9	& 18.495(0.080)	 & 17.833(0.041)	 & 17.412(0.025)	 & 17.280(0.025) \\ 
2003hk	  & 52905.47	 & 46.0	& 18.750(0.084)	 & 17.840(0.030)	 & 17.406(0.035)	 & 17.316(0.036) \\ 
2003hk	  & 52909.46	 & 50.0	& 19.055(0.112)	 & 17.945(0.036)	 & 17.452(0.019)	 & 17.330(0.036) \\ 
2003hk	  & 52912.48	 & 53.0	& 19.054(0.111)	 & 18.093(0.042)	 & 17.519(0.028)	 & 17.408(0.030) \\ 
2003hk	  & 52915.46	 & 56.0	& 19.223(0.103)	 & 18.079(0.042)	 & 17.570(0.023)	 & 17.400(0.037) \\ 
2003hk	  & 52918.44	 & 58.9	& 19.387(0.130)	 & 18.054(0.043)	 & 17.618(0.037)	 & 17.426(0.035) \\ 
2003hk	  & 52921.38	 & 61.9	& 19.675(0.157)	 & 18.177(0.071)	 & 17.576(0.034)	 & 17.433(0.051) \\ 
2003hk	  & 52927.39	 & 67.9	& 19.437(0.241)	 & 18.274(0.044)	 & 17.622(0.031)	 & 17.413(0.094) \\ 
2003hk	  & 52930.39	 & 70.9	& 19.722(0.249)	 & 18.238(0.050)	 & 17.700(0.033)	 & 17.524(0.053) \\ 
2003hk	  & 52934.38	 & 74.9	& 19.742(0.258)	 & 18.380(0.045)	 & 17.719(0.020)	 & 17.562(0.053) \\ 
2003hk	  & 52942.33	 & 82.8	& --	 & 18.732(0.072)	 & 17.852(0.064)	 & 17.705(0.063) \\ 
2003hk	  & 52947.31	 & 87.8	& --	 & 18.693(0.093)	 & 18.019(0.050)	 & 17.764(0.058) \\ 
2005dq	  & 53613.31	 & 5.2	& 17.355(0.019)	 & 17.483(0.042)	 & 17.474(0.028)	 & 17.358(0.056) \\ 
2005dq	  & 53614.32	 & 6.2	& 17.358(0.030)	 & 17.400(0.033)	 & 17.399(0.025)	 & 17.355(0.080) \\ 
2005dq	  & 53615.28	 & 7.2	& 17.417(0.023)	 & 17.421(0.039)	 & 17.365(0.022)	 & 17.214(0.059) \\ 
2005dq	  & 53617.27	 & 9.2	& 17.428(0.022)	 & 17.424(0.032)	 & 17.264(0.034)	 & 17.085(0.052) \\ 
2005dq	  & 53619.30	 & 11.2	& 17.462(0.026)	 & 17.463(0.038)	 & 17.248(0.028)	 & 17.052(0.050) \\ 
2005dq	  & 53623.26	 & 15.2	& 17.686(0.031)	 & 17.643(0.038)	 & 17.410(0.028)	 & 17.206(0.049) \\ 
2005dq	  & 53627.21	 & 19.1	& 17.980(0.057)	 & 17.788(0.047)	 & 17.694(0.035)	 & 17.382(0.050) \\ 
2005dq	  & 53633.34	 & 25.2	& 18.210(0.109)	 & 17.931(0.044)	 & 17.750(0.065)	 & 17.509(0.070) \\ 
2005dq	  & 53637.26	 & 29.2	& 18.537(0.078)	 & 18.164(0.063)	 & 17.814(0.062)	 & 17.518(0.097) \\ 
2005dq	  & 53641.22	 & 33.1	& 18.700(0.047)	 & 18.320(0.048)	 & 17.911(0.044)	 & 17.730(0.108) \\ 
2005dq	  & 53649.29	 & 41.2	& 19.151(0.071)	 & 18.349(0.067)	 & 18.102(0.039)	 & 17.812(0.145) \\ 
2005dq	  & 53650.23	 & 42.1	& 19.297(0.077)	 & 18.349(0.060)	 & 18.065(0.044)	 & 17.826(0.108) \\ 
2005dq	  & 53653.18	 & 45.1	& 19.322(0.065)	 & 18.534(0.147)	 & 18.144(0.074)	 & 17.739(0.141) \\ 
2005dq	  & 53657.20	 & 49.1	& 19.371(0.129)	 & 18.401(0.120)	 & 18.157(0.065)	 & 18.002(0.162) \\ 
2005dq	  & 53665.22	 & 57.1	& 19.555(0.113)	 & 18.585(0.072)	 & 18.225(0.075)	 & 17.933(0.051) \\ 
2005dq	  & 53669.19	 & 61.1	& 19.633(0.097)	 & 18.841(0.098)	 & 18.254(0.064)	 & 17.900(0.104) \\ 
2005dq	  & 53674.19	 & 66.1	& 19.651(0.083)	 & 18.961(0.095)	 & 18.279(0.079)	 & 18.000(0.094) \\ 
2005dq	  & 53678.13	 & 70.0	& --	 & 19.102(0.127)	 & 18.414(0.056)	 & 18.124(0.130) \\ 
2007fz	  & 54301.24	 & 5.1	& 16.959(0.017)	 & 16.679(0.014)	 & 16.498(0.016)	 & 16.364(0.018) \\ 
2007fz	  & 54303.19	 & 7.1	& 17.291(0.036)	 & 16.918(0.025)	 & 16.715(0.020)	 & 16.587(0.027) \\ 
2007fz	  & 54306.21	 & 10.1	& 17.530(0.037)	 & 17.142(0.025)	 & 16.880(0.020)	 & 16.783(0.035) \\ 
2007fz	  & 54308.19	 & 12.1	& 17.526(0.035)	 & 17.094(0.025)	 & 16.849(0.021)	 & 16.732(0.030) \\ 
2007fz	  & 54310.18	 & 14.1	& 17.459(0.052)	 & 17.074(0.032)	 & 16.777(0.026)	 & 16.679(0.023) \\ 
2007fz	  & 54312.18	 & 16.1	& 17.445(0.039)	 & --	 & 16.690(0.044)	 & 16.694(0.038) \\ 
2007fz	  & 54316.20	 & 20.1	& 17.620(0.035)	 & 17.012(0.021)	 & 16.684(0.015)	 & 16.645(0.030) \\ 
2007fz	  & 54319.20	 & 23.1	& --	 & 17.213(0.025)	 & 16.798(0.020)	 & 16.754(0.028) \\ 
2007fz	  & 54322.18	 & 26.1	& 18.457(0.045)	 & 17.566(0.033)	 & 17.057(0.029)	 & 16.899(0.039) \\ 
2007fz	  & 54325.17	 & 29.1	& 18.986(0.141)	 & 17.679(0.037)	 & 17.272(0.030)	 & 17.110(0.036) \\ 
2007fz	  & 54328.17	 & 32.1	& 18.849(0.129)	 & 18.016(0.043)	 & 17.462(0.038)	 & -- \\ 
2007fz	  & 54331.17	 & 35.1	& 19.387(0.122)	 & 18.206(0.050)	 & 17.619(0.029)	 & 17.344(0.075) \\ 
2007fz	  & 54334.17	 & 38.1	& 19.370(0.091)	 & 18.293(0.055)	 & 17.712(0.040)	 & 17.415(0.051) \\ 
2007fz	  & 54337.16	 & 41.1	& 19.439(0.252)	 & 18.592(0.121)	 & 17.811(0.050)	 & 17.601(0.052) \\ 
2007fz	  & 54340.16	 & 44.1	& --	 & 18.498(0.186)	 & 17.766(0.052)	 & 17.555(0.090) \\ 
2007fz	  & 54343.16	 & 47.1	& 19.466(0.159)	 & 18.649(0.114)	 & 17.913(0.042)	 & 17.727(0.068) \\ 
2007fz	  & 54346.15	 & 50.1	& --	 & 18.619(0.088)	 & 17.926(0.057)	 & 17.613(0.055) \\ 
2007fz	  & 54353.15	 & 57.1	& --	 & 18.737(0.094)	 & 18.108(0.057)	 & 17.731(0.048) \\ 
2007fz	  & 54359.14	 & 63.0	& --	 & 18.882(0.106)	 & 18.240(0.059)	 & 17.930(0.066) \\ 
2007fz	  & 54362.13	 & 66.0	& --	 & --	 & 18.333(0.057)	 & 17.827(0.067) \\ 
2007fz	  & 54368.13	 & 72.0	& --	 & --	 & --	 & 17.926(0.103) \\ 
2008es	  & 54616.24	 & 34.9	& --	 & --	 & 17.784(0.028)	 & 17.717(0.072) \\ 
2008es	  & 54618.26	 & 36.9	& --	 & --	 & 17.821(0.037)	 & 17.899(0.157) \\ 
2008es	  & 54620.22	 & 38.8	& 18.308(0.036)	 & 18.085(0.063)	 & 17.844(0.035)	 & 17.696(0.050) \\ 
2008es	  & 54622.23	 & 40.9	& 18.442(0.046)	 & 18.028(0.034)	 & 17.884(0.033)	 & 17.643(0.052) \\ 
2008es	  & 54624.22	 & 42.8	& 18.556(0.040)	 & --	 & 17.956(0.035)	 & 17.791(0.046) \\ 
2008es	  & 54626.22	 & 44.8	& 18.589(0.057)	 & 18.133(0.040)	 & 17.966(0.031)	 & 17.860(0.042) \\ 
2008es	  & 54628.22	 & 46.8	& 18.685(0.072)	 & 18.187(0.040)	 & 18.000(0.039)	 & 17.856(0.054) \\ 
2008es	  & 54630.22	 & 48.8	& 18.777(0.058)	 & 18.292(0.037)	 & 18.076(0.053)	 & 17.878(0.069) \\ 
2008es	  & 54632.24	 & 50.9	& 18.885(0.094)	 & 18.292(0.063)	 & 18.082(0.033)	 & 17.991(0.059) \\ 
2008es	  & 54634.27	 & 52.9	& 18.892(0.108)	 & 18.343(0.085)	 & 18.168(0.037)	 & 17.905(0.066) \\ 
2008es	  & 54636.23	 & 54.9	& 18.978(0.093)	 & 18.508(0.027)	 & 18.180(0.050)	 & 17.990(0.076) \\ 
2008es	  & 54639.20	 & 57.8	& 18.951(0.112)	 & 18.464(0.039)	 & 18.228(0.051)	 & 18.222(0.108) \\ 
2008es	  & 54643.24	 & 61.9	& 19.412(0.094)	 & 18.329(0.053)	 & 18.413(0.058)	 & 18.181(0.090) \\ 
2008fq	  & 54726.19	 & 6.4	& 16.281(0.900)	 & 15.707(0.900)	 & 15.418(0.900)	 & 15.141(0.900) \\ 
2008fq	  & 54728.21	 & 8.4	& --	 & 15.641(0.900)	 & 15.316(0.900)	 & 15.001(0.900) \\ 
2008fq	  & 54730.18	 & 10.4	& 16.359(0.900)	 & 15.637(0.900)	 & 15.257(0.900)	 & 14.948(0.900) \\ 
2008fq	  & 54732.21	 & 12.4	& 16.355(0.900)	 & 15.626(0.900)	 & 15.242(0.900)	 & 14.857(0.900) \\ 
2008fq	  & 54734.16	 & 14.4	& 16.434(0.900)	 & 15.642(0.900)	 & 15.206(0.900)	 & 14.833(0.900) \\ 
2008fq	  & 54736.16	 & 16.4	& 16.438(0.900)	 & 15.686(0.900)	 & 15.221(0.900)	 & 14.817(0.900) \\ 
2008fq	  & 54738.16	 & 18.4	& 16.555(0.900)	 & 15.718(0.900)	 & 15.259(0.900)	 & 14.835(0.900) \\ 
2008fq	  & 54740.17	 & 20.4	& 16.648(0.900)	 & 15.805(0.900)	 & 15.287(0.900)	 & 14.903(0.900) \\ 
2008fq	  & 54742.21	 & 22.4	& --	 & 15.907(0.900)	 & --	 & -- \\ 
2008fq	  & 54745.17	 & 25.4	& 16.925(0.900)	 & 16.020(0.900)	 & 15.342(0.900)	 & 15.059(0.900) \\ 
2008fq	  & 54750.15	 & 30.3	& 17.024(0.901)	 & 16.282(0.900)	 & 15.688(0.900)	 & 15.198(0.900) \\ 
2008fq	  & 54752.16	 & 32.4	& 17.362(0.900)	 & 16.336(0.900)	 & 15.726(0.900)	 & 15.265(0.900) \\ 
2008fq	  & 54754.14	 & 34.3	& 17.442(0.901)	 & 16.334(0.900)	 & 15.758(0.900)	 & 15.366(0.900) \\ 
2008fq	  & 54756.12	 & 36.3	& 17.516(0.900)	 & 16.401(0.900)	 & 15.791(0.900)	 & 15.382(0.900) \\ 
2008fq	  & 54758.13	 & 38.3	& 17.559(0.900)	 & 16.429(0.900)	 & 15.791(0.900)	 & 15.372(0.900) \\ 
2008fq	  & 54760.11	 & 40.3	& 17.611(0.900)	 & 16.480(0.900)	 & 15.821(0.900)	 & 15.402(0.900) \\ 
2008fq	  & 54763.12	 & 43.3	& 17.731(0.900)	 & 16.553(0.900)	 & 15.875(0.900)	 & 15.458(0.900) \\ 
2008fq	  & 54766.10	 & 46.3	& 17.784(0.901)	 & 16.630(0.900)	 & 15.849(0.900)	 & 15.454(0.900) \\ 
2008fq	  & 54781.09	 & 61.3	& 18.281(0.900)	 & 16.714(0.900)	 & 16.036(0.900)	 & 15.552(0.900) \\ 
2008fq	  & 54785.09	 & 65.3	& 18.236(0.900)	 & 16.846(0.900)	 & 16.105(0.900)	 & 15.621(0.900) \\ 
2008fq	  & 54789.09	 & 69.3	& 18.621(0.904)	 & 17.023(0.900)	 & 16.164(0.900)	 & 15.755(0.900) \\ 
\hline
\end{tabular}
\tablenotetext{a}{Days since explosion}
\end{table*}


==> spect2001cy.tex <==

 
\begin{table*}
\caption{Sample Journal of Spectroscopic Observations}
\begin{tabular}{cccccc}
\hline\hline
SN Name &
MJD &
Age (Days) \tablenotemark{a} &
Instrument &
Range (\AA)&
Exposure (s)\\
\hline
2001cy	 & 52106.48	 &21.5	 &Lick/Kast	 & 3300-10400 &900 \\ 
2001cy	 & 52117.42	 &32.4	 &Lick/Kast	 & 3300-10400 &900 \\ 
2001cy	 & 52144.45	 &59.4	 &Lick/Kast	 & 3300-10400 &900 \\ 
2001cy	 & 52164.25	 &79.2	 &Lick/Kast	 & 3300-10400 &900 \\ 
2001cy	 & 52172.32	 &87.3	 &Lick/Kast	 & 3300-10400 &900 \\ 
2001cy	 & 52207.12	 &122.1	 &Lick/Kast	 & 3280-10400 &1500 \\ 
...	 & ...	 &...	 &...	 & ...	 &... \\ 
\hline
\end{tabular}
\label{t:spec}
\tablenotetext{a}{Days since explosion}
\end{table*}

